Deductive Verification via the Debug Adapter Protocol

We propose a conceptual integration of deductive program verification into existing user interfaces for software debugging. This integration is well-represented in the "Debug Adapter Protocol", a widely-used and generic technology to integrate debugging of programs into development environments. Commands like step-forward and step-in are backed by steps of a symbolic structural operational semantics, and the different paths through a program are readily represented by multiple running threads of the debug target inside the user interface. Thus, existing IDEs can be leveraged for deductive verification debugging with relatively little effort. We have implemented this scheme for SecC, an auto-active program verifier for C, and discuss its integration into Visual Studio Code.

==> eptcsdata.tex <==
\providecommand{\firstpage}{89}
\providecommand{\publicationstatus}{A. Paskevich, J. Proen\c{c}a (Eds.): Formal Integrated\\
Development Environment 2021 (F-IDE 2021)\\
EPTCS 338, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.338.11}{10.4204/EPTCS.338.11}}
\pdfoutput=1

